MVSNeRF: Fast Generalizable Radiance Field Reconstruction from Multi-View Stereo

We present MVSNeRF, a novel neural rendering approach that can efficiently reconstruct neural radiance fields for view synthesis. Unlike prior works on neural radiance fields that consider per-scene optimization on densely captured images, we propose a generic deep neural network that can reconstruct radiance fields from only three nearby input views via fast network inference. Our approach leverages plane-swept cost volumes (widely used in multi-view stereo) for geometry-aware scene reasoning, and combines this with physically based volume rendering for neural radiance field reconstruction. We train our network on real objects in the DTU dataset, and test it on three different datasets to evaluate its effectiveness and generalizability. Our approach can generalize across scenes (even indoor scenes, completely different from our training scenes of objects) and generate realistic view synthesis results using only three input images, significantly outperforming concurrent works on generalizable radiance field reconstruction. Moreover, if dense images are captured, our estimated radiance field representation can be easily fine-tuned; this leads to fast per-scene reconstruction with higher rendering quality and substantially less optimization time than NeRF.

==> sec/method_backup.tex <==

\begin{figure*}[t]
\begin{center}
    \includegraphics[width=\linewidth]{LaTeX/fig/pipeline.pdf}
\end{center}
\caption{Pipeline of proposed MVSNeRF.}
\label{fig:pipeline}
\end{figure*}

\section{MVSNeRF}
Given neighbor source views $I_s$, our method attempts to synthesis high quality target view images $I_t$ without/with small amount feed-forward optimization. Unlike NeRF ~\cite{xxx} rendering free-viewpoint video (FVV) via a per-scene "network memory", our method borrow ideas from traditional image-based-rendering (IBR) methods ~\cite{xxx} that to learn a view interpolation rules from given nearby sampled view rendering, which enabling generalize our method to novel scenes. Our pipeline (Fig. ~\ref{fig:pipeline}) consistences three parts:  1) feature extraction and cost-volume construction, which extracting image feature from each source view and learns multi-view correspondences with 3D CNN based feature aggregation, and 2) rendering and regressing target images (RGB-$\sigma$) through a volumetric rendering scheme. Then, 3) we present how to rendering FVV from given any number of neighboring views in Sec. ~\ref{sec:Extension to novel scenes}.

In a nutshell, our complete novel view image rendering process can be formulate as:
\begin{equation}
I_t = \mathrm{MVSNeRF}(I_s, \mathcal{C}_s, \mathcal{C}_t) = \mathcal{R}(x, \mathbf{d}, f, \tilde{c})
\label{eq:mvsnerf}
\end{equation}

where $\mathcal R$ denotes the volumetric renderer which taking normalized device coordinates (NDC) $x \in \mathbb{R}^3 \ | \ x = z \mathbf{d}$ with depth $z$, ray directions $\mathbf{d}$ under referent view space, volume features $f$ and skip color connection $\widetilde{c}$ as input. More specifically,

\begin{equation}
 f = \mathcal{G}(x, Cost(I_s, \mathcal{C})); \ \tilde{c} = \mathcal{G}(\mathcal{H}(x, \mathcal{C}), I_s)
\label{eq:mvsnerf_notation}
\end{equation}



$\mathcal{C} = [R,T,K]$ stands for the source and target camera poses modeling with three dimensional rotation $R$, translation $T$ and intrinsic $K$. $\mathcal{G}$ is a linear grid interpolation operation inside the convolved cost-volume and $\mathcal{H}$ is homograph wrapping from volume points to source image plan.



\subsection{Feature extraction and Cost-volume construction}

\textbf{Extracting image feature.} Instead of representing entry scenes, our method attempts to learn local radiance fields from fixing number (e.g., $3$ views in experiment) of source images $\textbf{I}^i_s \in \mathbb{R}^{H_i \times W_i \times 3}, i \in [1,2,3]$, similar to most image process tasks, we extract image feature $\textbf{F}_i \in \mathbb{R}^{H_i/4 \times W_i/4 \times C} $ with shared 2D CNN layers to capture multi-level information for the following regression phase. 

\textbf{Learning multi-view correspondences: Cost-Volume}
Given referent views and their feature maps, we set up to build a cost volume that include epipolar geometric constant and resolve 3D geometric ambiguities . Unlike most neural scene representations learn geometric constant via Markov process ~\cite{NeRF like}, or point feature matching ~\cite{GRF, pixelnerf, ibrnet} (i.e., indexing and aggregating sample points' features via a projection scheme). The continuity of neighboring points aren't welly represented and explored, thus we 
apply two volumes cost-volume and feature volume for surface radiance and geometric modeling, which are build on referent camera space, as shown in Fig.~\ref{fig:pipeline}. 

We borrow the cost volume idea from multi-view stereo matching networks ~\cite{xxx} and further to extent it to a continue volume with a unsupervised volume rendering scheme. Similar to previous multi-view stereo matching networks, we utilize plane hypothesis to compute a cost variance volume from the extracted feature maps,

\begin{equation}
\begin{aligned}
    \mathcal{H}_i(t) = K_i \cdot( R_i \cdot R_1^T + \frac{(t_1-t_i)\cdot n^{T}_1}{z}) \cdot K^{-1}_{1}
\label{eq:homograph}
\end{aligned}
\end{equation}
where $\mathcal{H}_i(z)$ refers to the homograph between the feature maps of the $i^{th}$ view and the reference view at depth $z$, $K_i, R_i, t_i$ denote the camera intrinsic/rotation/translation matrix respectively and $n_1$ is the look-at direction of the reference camera. Note that, we use referent view coordinate system instead of  canonical coordinate frame in NeRF like representations, since no clear canonical coordinate system exists on scenes with multiple objects or real scenes.

Thereby, we build a perspective cost volume grid $PCV$ to modeling the scene (as shown in the middle of Fig.~\ref{xxx}). Feature $f_p$ of each grid point $p(u,v,z) \in \mathbb{R}^3$ is aggregated as,

\begin{equation}
\begin{aligned}
    PCV(p) &= f_p = \frac{1}{n} <f^1_p, ..., f^m_p>\\
    f^i_p &= \mathcal{G}( F_i, H_i(z) \cdot [u,v,1]^T)
\label{eq:cost volume}
\end{aligned}
\end{equation}
where $<,>$ denotes the inner product between source view features under the same grid point $p$, while $m$ is the number of the sources views and $m=3$ in our experiment.

Next, we adopt a 3D CNN on the cost volume to matching features and explicitly enforce neighboring volume points share contents. However, 3D CNN on the grid points couldn't guarantee volume continuity and usually result in the well-known edge-fattening issue in MVSNets, to address this issue, we propose to use a volume rendering scheme after the 3D CONV, which enable preserving the volume continuity.

\subsection{Rendering Images}
\textbf{Predicting RGB-$\sigma$}
Our method synchronously optimize geometric and radiance field with the classical volume rendering: accumulating colors and densities along rays to render image. Unlike NeRF-like methods ~\cite{nerf} modelling a continue scene as a $5D$ vector-valued functions, which taking $3D$ position $p$ and $2D$ viewing direction $(\theta,\phi)$ as inputs. Since geometric and radiance fields can be varying across scenes, coordinate-based function mapping lacking the generalizationbility, we extend the classical $5D$ coordinate inputs with convolved volume feature  $f \in \mathbb{R}^{M}$ and color $c \in \mathbb{R}^{n \times 3}$ to handle scene specify information:

\begin{equation}
    \mathcal{R}(\mathbf{r}) = \int_{t_n}^{t_f}T(t)\sigma(t)\textbf{c}(t)dt
\end{equation}


Where $\mathbf{r} = (x,\mathbf{d}, f, c)$ is point samples along the ray direction, $T(t) = exp(-\int_{t_n}^{t}\sigma(\textbf{r}(s))ds)$ is the "cumproded" density along the ray from $t_n$ to $t$, while the $\mathbf{c},\sigma$ is the RGB and density of the given spacial point $\mathbf{x}$ its direction $\mathbf{d}$ toward to  viewpoint. Under this modeling, target views can be obtained by casting rays to the volume and thus we can easily regressive the scene via a differential rendering scheme.


\textbf{Training Objective.}
Since our cost volume construction and volume renderer are fully differentiable, our MVSNeRF can optimize end-to-end. For each iteration, We sample $4$ pair-wised neighboring images from training set and use $3$ of them to construct cost volume and the lefr one as target view. We sample rays emitting from the target view and minimize the mean squared error between the rendered colors and ground truth pixel colors for training:

\begin{equation}
     \mathcal{L} = \sum_{\mathbf{r} \in R} || I_t^\mathbf{r} - \mathcal{R}(\mathbf{r}) ||^2
\end{equation}

\textbf{Soft volume fusion.} Rendering novel view only from single local metric inevitably lead to artifacts on such occlusion areas, thus it is naturally predict target images by fusing neighboring local volumes. Instead of directly fusing final rendering results obtained from nearby volumes or average pooling in feature space ~\cite{pixelnerf}. We propose an explicit weighting function that softly fuse nearby local volumes in feature space, and fine-tuning the network by fixing the weight function to ensure that the space is interpolable.

First, we build $m$ $PCV$ from $m$ source view images with Eq.~\ref{eq:cost volume}. Then, we present a fusion scheme analogous to unstructured lumigraph \cite{buehler2001unstructured}, that adaptively modify the weights according to visibility, the angular distance between the novel view and the source volumes. For each volume point $x$, the weight of $i_{th}$ volume as:

\begin{equation}
\begin{aligned}
w_i = \frac{ \tau_i \cdot e^{-\alpha \cdot (1.0  + n_i \cdot \mathbb{d})}}{\sum_{i=1}^{m}  \tau_i \cdot e^{-\alpha \cdot (1.0  + n_i \cdot \mathbb{d})}}
\end{aligned}
\end{equation}

where $m$ denotes the number views, $n_i$ is the lookat direction of $i_{th}$ source view and $\tau_i \in [0.0,1.0]$ is the one-hot label that determine the sample point $x$ whether inside the referent volume $i$. $\alpha$ is a hyperparameter, we set $30$ in our experiment.

Finally, we fine-tuning the network by fixing the weighting function.

\subsection{Extension to any number of nearby views}
\label{sec:Extension to novel scenes}

Furthermore, it's naturally to extend our framework to allow for an arbitrary number of views at training or testing time, thus can prove additional information about the scene and enabling to render larger free viewpoint image baseline. To this end, we can render each target view with two ways: 1) volume interpolation between the source local volumes, or 2) fine tuning the network to better represent the specify scene from the pre-trained modules. Before the interpolation and fine-tuning, we need to select the referent views for each target view.


\begin{figure}[t]
\begin{center}
    \includegraphics[width=\linewidth]{LaTeX/fig/view_seletion.pdf}
\end{center}
\caption{xxx}
\label{fig:view_seletion}
\end{figure}

\textbf{Referent View selection.} Given multiply neighboring source views $I_s$ and the pose of target virtual view $[R_t,t]$, we  select $3$ reference views  base on its position and lookat direction. As mentioned in the above sections, our pipeline take $3$ neighboring images for the cost volume construction and radiance field rendering in training stage. Note that our cost volume construction is not limited by the input view number since the inner product operation in Eq.~\ref{eq:cost volume} is  order and number free, thus we can use multiply input views for a better cost volume construction, and select three specific views for the  color skipping (i.e., xx line of Fig. ~\ref{xx}).

To better recover target views, we propose a view triangulation scheme to make sure the pair-wised referent views are include as much radiance information as required. As shown in Fig~\ref{xxx}, we first select $V^i_p, i \in [1,M]$ and $V^l_l, i \in [1,N]$ nearest views via the position and lookat-angle distance respectively. Next, we used the first $K$ intersection views as the referent view candidates, i.e. $V_p \cap V_l$.  Furthermore, we pair the view candidates condition on the target view is "inside" the triangles formed with referent view position, as (b) of Fig.~\ref{xxx}. We project the camera position of candidate views to the camera space of the target view with their extrinsic parameters and classify each camera into its' azimuth:

\begin{equation}
\begin{aligned}
    C(p) &= f_p = \frac{1}{3} <f^1_p, f^2_p, f^3_p>\\
    f^i_p &= \mathcal{G}( F_i, H_i(d) \cdot [x,y,1]^T)
\label{eq:view selection}
\end{aligned}
\end{equation}

Next, we group the cameras inside bin $0,2,4$ and $1,3,5$ to be the referent pairs that can make sure target view are "inside" Referent-View-Triangles and thus can significant avoid the artifacts cased by occlusion (demonstrated in Appendix). 


\textbf{Fine-tuning.}
By combining the above Soft volume fusion and referent view selection, we can achieve large baseline or even $360^\circ$ free viewpoint rendering just from the pre-train models on large scale dataset. However, ghosting artifacts and blurry edges  are generally observed when view changing due to the limited compatibility of the trained models. Thus, we include a small number of feed-forward optimization on the input views. Instead of using local ray direction and NDC position in the previous sections, we use global scene coordinate when optimizing on a specify scene. Fine-tuning only on a specific scene with scene coordinate can improve  performance on view consistence, geometric and radiance.

==> sec/overview.tex <==
\section{Overview}
